An Implementation of the Quantum Verification of Matrix Products Algorithm

We present a space-efficient implementation of the quantum verification of matrix products (QVMP) algorithm and demonstrate its functionality by running it on the Aer simulator with two simulation methods: statevector and matrix product state (MPS). We report circuit metrics (gate count, qubit count, circuit depth), transpilation time, simulation time, and a proof of Grover oracle correctness. Our study concludes that while QVMP can be simulated on moderately sized inputs, it cannot scale to a degree where we can observe any quantum advantage on current quantum hardware due to circuit depth and qubit count constraints. Further, the choice of simulation method has a noticeable impact on the size of the transpiled circuit which slows down development.

==> tables/circuit_metrics_isca.tex <==
\begin{table*}
    \centering
    \begin{subtable}{\textwidth}
      \resizebox{\textwidth}{!}{%
        \begin{tabular}{|l|c||c|c|c|c|c|c|c|c||c|c|c|c|}
          \hline
          Dimension & Mismatches & ccx &      cx &   x &     h & z &      u1 &    u2 & u3 & Grover iterations &   Depth & Qubits & Total gates \\
          \hline
           (4, 4) &          1 &  30 &       1 &  11 &     2 & 1 &       2 &     2 &  0 &                 1 &      44 &     11 &          49 \\
          (16, 8) &          2 &  32 &   10108 &  69 &   284 & 2 &    8460 &  2536 &  3 &                 2 &   16993 &     21 &       21494 \\
          (32, 8) &          1 &  64 &   91408 & 272 &   997 & 4 &   91377 &  1056 &  8 &                 4 &  150375 &     22 &      185186 \\
         (32, 32) &          3 & 128 &  185912 & 151 &  2025 & 2 &  185897 &  2052 &  4 &                 2 &  303901 &     70 &      376171 \\
         (64, 16) &          2 & 128 &  786960 & 538 &  4190 & 4 &  786948 &  4232 &  5 &                 4 & 1300351 &     39 &     1583005 \\
         (64, 64) &          3 & 384 & 2329596 & 432 & 12396 & 3 & 2329587 & 12426 &  4 &                 3 & 3843672 &    135 &     4684828 \\
          \hline
        \end{tabular}}
      \caption{MPS}
      \label{table:circuit_metrics_mps}
    \end{subtable}
    \begin{subtable}{\textwidth}
      \resizebox{\textwidth}{!}{%
        \begin{tabular}{|l|c||c|c|c|c|c|c|c|c||c|c|c|c|}
          \hline
          Dimension & Mismatches & ccx &      cx &   x &     h & z &      u1 &    u2 & u3 & Grover iterations &   Depth & Qubits & Total gates \\
          \hline
          (4, 4) &          1 &  30 &  1 &  11 & 2 & 1 &  2 &  2 &  0 &                 1 &    44 &     11 &          49 \\
         (16, 4) &          2 &  16 &  0 &  75 & 4 & 2 &  3 & 12 &  1 &                 2 &   261 &     13 &         113 \\
         (16, 8) &          2 &  32 &  0 &  76 & 4 & 2 &  3 & 12 &  1 &                 2 &   385 &     21 &         130 \\
         (32, 4) &          2 &  24 &  0 & 208 & 5 & 3 &  4 & 24 &  2 &                 3 &   684 &     14 &         270 \\
         (64, 8) &          3 &  48 &  0 & 405 & 6 & 3 &  4 & 30 &  2 &                 3 &  2040 &     23 &         498 \\
         (64, 8) &          1 &  96 &  0 & 801 & 6 & 6 &  7 & 60 &  5 &                 6 &  4077 &     23 &         981 \\
          \hline
        \end{tabular}}
      \caption{Statevector}
      \label{table:circuit_metrics_statevector_cpu}
    \end{subtable}
    \caption{Circuit metrics for MPS and statevector simulation methods on
    select dimensions. Depth and total gates were measured after transpilation.}
    \label{table:circuit_metrics}
  \end{table*}


==> tables/circuit_metrics_mps.tex <==
\begin{tabular}{|c|c||c|c|c|c|c|c|c|c||c|c|c|c|}
\toprule
Dimension & Mismatches & ccx &      cx &   x &     h & z &      u1 &    u2 & u3 & Grover iterations &   Depth & Qubits & Total gates \\
\midrule
   (4, 2) &          0 &  18 &       1 &  11 &     2 & 1 &       2 &     2 &  0 &                 1 &      32 &      7 &          37 \\
   (4, 2) &          1 &  16 &       1 &  11 &     2 & 1 &       2 &     2 &  0 &                 1 &      30 &      7 &          35 \\
   (4, 2) &          2 &   0 &       0 &   1 &     2 & 0 &       0 &     0 &  0 &                 0 &       2 &      7 &           3 \\
   (4, 2) &          3 &   0 &       0 &   1 &     2 & 0 &       0 &     0 &  0 &                 0 &       2 &      7 &           3 \\
   (4, 4) &          0 &  28 &       1 &  11 &     2 & 1 &       2 &     2 &  0 &                 1 &      42 &     11 &          47 \\
   (4, 4) &          1 &  30 &       1 &  11 &     2 & 1 &       2 &     2 &  0 &                 1 &      44 &     11 &          49 \\
   (4, 4) &          2 &   0 &       0 &   1 &     2 & 0 &       0 &     0 &  0 &                 0 &       2 &     11 &           3 \\
   (4, 4) &          3 &   0 &       0 &   1 &     2 & 0 &       0 &     0 &  0 &                 0 &       2 &     11 &           3 \\
  (16, 4) &          0 &   8 &    2966 &  37 &    86 & 1 &    2488 &   746 &  2 &                 1 &    5058 &     13 &        6334 \\
  (16, 4) &          1 &  24 &    9114 &  99 &   256 & 3 &    7644 &  2292 &  4 &                 3 &   15522 &     13 &       19436 \\
  (16, 4) &          2 &  16 &    6220 &  68 &   176 & 2 &    5216 &  1564 &  3 &                 2 &   10585 &     13 &       13265 \\
  (16, 4) &          3 &   8 &    3182 &  37 &    92 & 1 &    2668 &   800 &  2 &                 1 &    5412 &     13 &        6790 \\
  (16, 8) &          0 &  16 &    5198 &  38 &   148 & 1 &    4350 &  1304 &  2 &                 1 &    8734 &     21 &       11057 \\
  (16, 8) &          1 &  48 &   15378 & 100 &   430 & 3 &   12870 &  3858 &  4 &                 3 &   25842 &     21 &       32691 \\
  (16, 8) &          2 &  32 &   10108 &  69 &   284 & 2 &    8460 &  2536 &  3 &                 2 &   16993 &     21 &       21494 \\
  (16, 8) &          3 &  16 &    5126 &  38 &   146 & 1 &    4290 &  1286 &  2 &                 1 &    8616 &     21 &       10905 \\
 (16, 16) &          0 &  32 &    8510 &  45 &   240 & 1 &    7110 &  2132 &  2 &                 1 &   14178 &     37 &       18072 \\
 (16, 16) &          1 &  96 &   28338 & 104 &   790 & 3 &   23670 &  7098 &  4 &                 3 &   47130 &     37 &       60103 \\
 (16, 16) &          2 &  64 &   17020 &  76 &   476 & 2 &   14220 &  4264 &  3 &                 2 &   28353 &     37 &       36125 \\
 (16, 16) &          3 &  32 &    8582 &  45 &   242 & 1 &    7170 &  2150 &  2 &                 1 &   14296 &     37 &       18224 \\
  (32, 4) &          0 &   8 &   14388 &  72 &   161 & 1 &   14381 &   172 &  2 &                 1 &   23772 &     14 &       29185 \\
  (32, 4) &          1 &  32 &   56816 & 270 &   621 & 4 &   56785 &   680 &  8 &                 4 &   93879 &     14 &      115216 \\
  (32, 4) &          2 &  24 &   42060 & 204 &   461 & 3 &   42037 &   504 &  6 &                 3 &   69510 &     14 &       85299 \\
  (32, 4) &          3 &  16 &   27672 & 138 &   305 & 2 &   27657 &   332 &  4 &                 2 &   45741 &     14 &       56126 \\
  (32, 8) &          0 &  16 &   22668 &  74 &   251 & 1 &   22661 &   262 &  2 &                 1 &   37296 &     22 &       45935 \\
  (32, 8) &          1 &  64 &   91408 & 272 &   997 & 4 &   91377 &  1056 &  8 &                 4 &  150375 &     22 &      185186 \\
  (32, 8) &          2 &  48 &   69108 & 206 &   755 & 3 &   69085 &   798 &  6 &                 3 &  113682 &     22 &      140009 \\
  (32, 8) &          3 &  32 &   46440 & 140 &   509 & 2 &   46425 &   536 &  4 &                 2 &   76389 &     22 &       94088 \\
 (32, 16) &          0 &  32 &   48060 &  74 &   527 & 1 &   48053 &   538 &  2 &                 1 &   78720 &     38 &       97287 \\
 (32, 16) &          1 & 128 &  191504 & 272 &  2085 & 4 &  191473 &  2144 &  8 &                 4 &  313671 &     38 &      387618 \\
 (32, 16) &          2 &  96 &  144180 & 206 &  1571 & 3 &  144157 &  1614 &  6 &                 3 &  236154 &     38 &      291833 \\
 (32, 16) &          3 &  64 &   96488 & 140 &  1053 & 2 &   96473 &  1080 &  4 &                 2 &  158037 &     38 &      195304 \\
 (32, 32) &          0 &  64 &   93140 &  85 &  1017 & 1 &   93133 &  1028 &  2 &                 1 &  152252 &     70 &      188470 \\
 (32, 32) &          1 & 256 &  371824 & 283 &  4045 & 4 &  371793 &  4104 &  8 &                 4 &  607799 &     70 &      752317 \\
 (32, 32) &          2 & 192 &  278316 & 217 &  3029 & 3 &  278293 &  3072 &  6 &                 3 &  454950 &     70 &      563128 \\
 (32, 32) &          3 & 128 &  185912 & 151 &  2025 & 2 &  185897 &  2052 &  4 &                 2 &  303901 &     70 &      376171 \\
  (64, 8) &          0 &  16 &  100484 & 139 &   540 & 1 &  100481 &   546 &  2 &                 1 &  166346 &     23 &      202209 \\
  (64, 8) &          1 &  96 &  600648 & 794 &  3198 & 6 &  600630 &  3264 &  7 &                 6 &  994341 &     23 &     1208643 \\
  (64, 8) &          2 &  64 &  398928 & 532 &  2126 & 4 &  398916 &  2168 &  5 &                 4 &  660415 &     23 &      802743 \\
  (64, 8) &          3 &  48 &  300324 & 401 &  1602 & 3 &  300315 &  1632 &  4 &                 3 &  497172 &     23 &      604329 \\
 (64, 16) &          0 &  32 &  197492 & 145 &  1056 & 1 &  197489 &  1062 &  2 &                 1 &  326330 &     39 &      397279 \\
 (64, 16) &          1 & 192 & 1182696 & 800 &  6294 & 6 & 1182678 &  6360 &  7 &                 6 & 1954245 &     39 &     2379033 \\
 (64, 16) &          2 & 128 &  786960 & 538 &  4190 & 4 &  786948 &  4232 &  5 &                 4 & 1300351 &     39 &     1583005 \\
 (64, 16) &          3 &  96 &  591348 & 407 &  3150 & 3 &  591339 &  3180 &  4 &                 3 &  977124 &     39 &     1189527 \\
 (64, 32) &          0 &  64 &  393012 & 154 &  2096 & 1 &  393009 &  2102 &  2 &                 1 &  648762 &     71 &      790440 \\
 (64, 32) &          1 & 384 & 2355816 & 809 & 12534 & 6 & 2355798 & 12600 &  7 &                 6 & 3888837 &     71 &     4737954 \\
 (64, 32) &          2 & 256 & 1572048 & 547 &  8366 & 4 & 1572036 &  8408 &  5 &                 4 & 2595039 &     71 &     3161670 \\
 (64, 32) &          3 & 192 & 1180164 & 416 &  6282 & 3 & 1180155 &  6312 &  4 &                 3 & 1948140 &     71 &     2373528 \\
 (64, 64) &          0 & 128 &  777660 & 170 &  4142 & 1 &  777657 &  4148 &  2 &                 1 & 1283086 &    135 &     1563908 \\
 (64, 64) &          1 & 768 & 4663704 & 825 & 24810 & 6 & 4663686 & 24876 &  7 &                 6 & 7694781 &    135 &     9378682 \\
 (64, 64) &          2 & 512 & 3107632 & 563 & 16534 & 4 & 3107620 & 16576 &  5 &                 4 & 5127375 &    135 &     6249446 \\
 (64, 64) &          3 & 384 & 2329596 & 432 & 12396 & 3 & 2329587 & 12426 &  4 &                 3 & 3843672 &    135 &     4684828 \\
\bottomrule
\end{tabular}


==> tables/circuit_metrics_statevector_cpu.tex <==
\begin{tabular}{|c|c||c|c|c|c|c|c|c|c||c|c|c|c|}
\toprule
Dimension & Mismatches & ccx & cx &   x & h & z & u1 & u2 & u3 & Grover iterations & Depth & Qubits & Total gates \\
\midrule
   (4, 2) &          0 &  18 &  1 &  11 & 2 & 1 &  2 &  2 &  0 &                 1 &    32 &      7 &          37 \\
   (4, 2) &          1 &  16 &  1 &  11 & 2 & 1 &  2 &  2 &  0 &                 1 &    30 &      7 &          35 \\
   (4, 2) &          2 &   0 &  0 &   1 & 2 & 0 &  0 &  0 &  0 &                 0 &     2 &      7 &           3 \\
   (4, 2) &          3 &   0 &  0 &   1 & 2 & 0 &  0 &  0 &  0 &                 0 &     2 &      7 &           3 \\
   (4, 4) &          0 &  28 &  1 &  11 & 2 & 1 &  2 &  2 &  0 &                 1 &    42 &     11 &          47 \\
   (4, 4) &          1 &  30 &  1 &  11 & 2 & 1 &  2 &  2 &  0 &                 1 &    44 &     11 &          49 \\
   (4, 4) &          2 &   0 &  0 &   1 & 2 & 0 &  0 &  0 &  0 &                 0 &     2 &     11 &           3 \\
   (4, 4) &          3 &   0 &  0 &   1 & 2 & 0 &  0 &  0 &  0 &                 0 &     2 &     11 &           3 \\
  (16, 4) &          0 &   8 &  0 &  41 & 4 & 1 &  2 &  6 &  0 &                 1 &   128 &     13 &          62 \\
  (16, 4) &          1 &  24 &  0 & 109 & 4 & 3 &  4 & 18 &  2 &                 3 &   384 &     13 &         164 \\
  (16, 4) &          2 &  16 &  0 &  75 & 4 & 2 &  3 & 12 &  1 &                 2 &   261 &     13 &         113 \\
  (16, 4) &          3 &   8 &  0 &  41 & 4 & 1 &  2 &  6 &  0 &                 1 &   134 &     13 &          62 \\
  (16, 8) &          0 &  16 &  0 &  42 & 4 & 1 &  2 &  6 &  0 &                 1 &   198 &     21 &          71 \\
  (16, 8) &          1 &  48 &  0 & 110 & 4 & 3 &  4 & 18 &  2 &                 3 &   582 &     21 &         189 \\
  (16, 8) &          2 &  32 &  0 &  76 & 4 & 2 &  3 & 12 &  1 &                 2 &   385 &     21 &         130 \\
  (16, 8) &          3 &  16 &  0 &  42 & 4 & 1 &  2 &  6 &  0 &                 1 &   196 &     21 &          71 \\
  (32, 4) &          0 &   8 &  0 &  74 & 5 & 1 &  2 &  8 &  0 &                 1 &   234 &     14 &          98 \\
  (32, 4) &          1 &  32 &  0 & 275 & 5 & 4 &  5 & 32 &  3 &                 4 &   919 &     14 &         356 \\
  (32, 4) &          2 &  24 &  0 & 208 & 5 & 3 &  4 & 24 &  2 &                 3 &   684 &     14 &         270 \\
  (32, 4) &          3 &  16 &  0 & 141 & 5 & 2 &  3 & 16 &  1 &                 2 &   453 &     14 &         184 \\
  (32, 8) &          0 &  16 &  0 &  76 & 5 & 1 &  2 &  8 &  0 &                 1 &   332 &     22 &         108 \\
  (32, 8) &          1 &  64 &  0 & 277 & 5 & 4 &  5 & 32 &  3 &                 4 &  1327 &     22 &         390 \\
  (32, 8) &          2 &  48 &  0 & 210 & 5 & 3 &  4 & 24 &  2 &                 3 &  1002 &     22 &         296 \\
  (32, 8) &          3 &  32 &  0 & 143 & 5 & 2 &  3 & 16 &  1 &                 2 &   673 &     22 &         202 \\
  (64, 8) &          0 &  16 &  0 & 141 & 6 & 1 &  2 & 10 &  0 &                 1 &   684 &     23 &         176 \\
  (64, 8) &          1 &  96 &  0 & 801 & 6 & 6 &  7 & 60 &  5 &                 6 &  4077 &     23 &         981 \\
  (64, 8) &          2 &  64 &  0 & 537 & 6 & 4 &  5 & 40 &  3 &                 4 &  2711 &     23 &         659 \\
  (64, 8) &          3 &  48 &  0 & 405 & 6 & 3 &  4 & 30 &  2 &                 3 &  2040 &     23 &         498 \\
\bottomrule
\end{tabular}

